A Deadline-Aware Scheduler for Smart Factory using WiFi 6

A key strategy for making production in factories more efficient is to collect data about the functioning of machines, and dynamically adapt their working. Such smart factories have data packets with a mix of stringent and non-stringent deadlines with varying levels of importance that need to be delivered via a wireless network. However, the scheduling of packets in the wireless network is crucial to satisfy the deadlines. In this work, we propose a technique of utilizing IEEE 802.11ax, popularly known as WiFi 6, for such applications. IEEE 802.11ax has a few unique characteristics, such as specific configurations of dividing the channels into resource units (RU) for packet transmission and synchronized parallel transmissions. We model the problem of scheduling packets by assigning profit to each packet and then maximizing the sum of profits. We first show that this problem is strongly NP-Hard, and then propose an approximation algorithm with a 12-approximate algorithm. Our approximation algorithm uses a variant of local search to associate the right RU configuration to each packet and identify the duration of each parallel transmission. Finally, we extensively simulate different scenarios to show that our algorithm works better than other benchmarks.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> algo-old.tex <==
\section{An Optimal Algorithm for the Scheduling Problem}
\label{sec:optimal}

\noindent The scheduling problem defined earlier can be mapped to the problem of finding the Maximum Weighted Matching in an Undirected Bipartite Graph. A matching in an undirected graph is a set of edges with no common vertices. Optimal algorithms for solving the Maximum Weighted Bipartite Matching problem are well known, and take almost linear time $O(n^{2}logn + ne)$ to execute.

\subsection{Mapping Procedure}

We now describe the mapping procedure between our scheduling problem and the Maximum Weighted Bipartite Matching problem.

\begin{figure}[t]
  \centering
    \includegraphics[width = 0.5\textwidth]{figs/max_weight_matching.pdf}
    \caption{Graph Constructed by Minimize Deadline Profit Scheduler}
    \label{fig:max_matching}
\end{figure}

\noindent As an input to our scheduling problem, we are given the set $C_{s} = \{ <T_{0}, s_{0}, d_{0}, P_{0}>, <T_{1}, s_{1}, d_{1}, P_{1}>, \dots <T_{l-1}, s_{l-1}, d_{l-1}, P_{l-1}> \}$ that describes the $l$ wireless applications $A_{s} = \{ A_{0}, A_{1}, \dots A_{l-1} \}$ in our factory setting, and a fixed RU configuration containing $j$ equal sized RUs.

\begin{algorithm}
def OptimalMinimizeDeadlineProfitScheduling($C_{s}$, $A_{s}$, $j$, $t_{i}$):\\
\>$n = LCM$ ($T_{0}, T_{1}, \dots T_{l-1}$) $- 1$\\
\>Create $t_{s} = \{ t_{i}, t_{i+1}, \dots t_{i+n-1} \}$\\
\>$m = \sum_{i} n+1 / T_{i}$\\
\>Create $p_{s} = \{ p_{0}, p_{1}, \dots p_{m-1} \}$\\
\>\\
\>$G = <V_{1} \cup V_{2}, E, W> = $ ConstructBipartiteNullGraph($m$, $n*j$)\\
\>\\
\>for each $A \in A_{s}$:\\
\>\>\>\>for each $p \in p_{s}$:\\
\>\>\>\>\>\>\>for each $t \in t_{s}$:\\
\>\>\>\>\>\>\>\>\>\>if $t \in [a_{Ap}, d_{Ap}]$:\\
\>\>\>\>\>\>\>\>\>\>for each $r \in r_{s}$:\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$u_{Ap} = V_{1}.$find($A, p$)\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$v_{tr} = V_{2}.$find($t, r$)\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$E$.add($u_{Ap}, v_{tr}$)\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$W$.add($u_{Ap}, v_{tr}$, $P_{A}$)\\
\>\\
\>$E^{'} = $ MaximumWeightedBipartiteMatching($G$)\\
\>\\
\>return $E^{'}$\\
\caption{Optimal Minimize Deadline Profit Scheduling Algorithm}\label{al:1}
\end{algorithm}

\noindent Based on the time periods of packet arrival for the different applications, $T_{0}, T_{1}, \dots T_{l-1}$, it evident that the pattern of packet arrival repeats are every $n+1 = LCM$ ($T_{0}, T_{1}, \dots T_{l-1}$) time instants.

\noindent Moreover, application $A_{i}$ generates $n+1 / T_{i}$ packets before its packet arrival pattern repeats at time instant $t_{i+n+1}$. Hence, over $n$ time instants $t_{s} = \{ t_{i}, t_{i+1}, \dots t_{i+n-1} \}$, total $m = \sum_{i} n+1 / T_{i}$ packets $p_{s} = \{ p_{0}, p_{1}, \dots p_{m-1} \}$ arrive. And for each time instant, we have $j$ equal sized RUs available $r_{s} = \{ r_{0}, r_{1} \dots r_{j-1} \}$.

\noindent We construct the weighted undirected bipartite graph $G = <V_{1} \cup V_{2}, E, W>$ such that, $|V_{1}| = m$ and $|V_{2}| = n*j$ shown in Figure \ref{fig:max_matching}. That is, the nodes in $V_{1}$ represents packets and the nodes in $V_{2}$ represent available RUs at different time instants.

\noindent A node $u_{Ap}$ $\epsilon$ $V_{1}$ represents the $p^{th}$ packet of the $A^{th}$ application. Similarly, a node $v_{tr}$ $\epsilon$ $V_{2}$ represents the $r^{th}$ RU available at the time instant $t$. Also, $[a_{Ap}, d_{Ap}]$ denotes the time window in which the $p^{th}$ packet of the $A^{th}$ application can be scheduled, since $a_{Ap}$ is the arrival time of the packet and $d_{Ap}$ is the deadline of the packet.

\noindent Then, in graph $G$, $\exists$ $(u_{Ap}, v_{tr}) 
\in E$ if and only if $t \in [a_{Ap}, d_{Ap}]$.

\noindent That is, if the $p^{th}$ packet of the $A^{th}$ application is available for scheduling in the time window $[a_{Ap}, d_{Ap}]$, then there would be an edge from $u_{Ap}$ in $V_{1}$ to all $v_{tr}$ in $V_{2}$ where $t$ $\epsilon$ $[a_{Ap}, d_{Ap}]$. Hence, if a packet arrives at time instant $t_{0}$ and has a deadline at time instant $t_{n}$, then there would be an edge from the node corresponding to the packet in $V_{1}$ to \textit{every} node in $V_{2}$. On the other hand, if the packet arrives in $t_{0}$ and has the deadline in $t_{0}$ itself, then there would be an edge from the packet's node to the nodes $v_{00}, v_{01}, \dots v_{0j}$ $\epsilon$ $V_{2}$, given that $j$ RUs are available. For example, in Figure \ref{fig:max_matching} packet $u_{10} \in V_{1}$ arrives at time instant $t_{0}$ and has a deadline at $t_{1}$, so there is an edge from $u_{10}$ to $v_{00}, v_{01}, \dots v_{13}$ reflecting the fact that $u_{10}$ can be assigned any available RU in those two time instants. 

\noindent Finally, $\forall$ $(u_{Ap}, v_{tr})$ $\epsilon$ $E$, we assign a weight $P_{A}$ which represents the profit/priority associated with each packet of the $A^{th}$ application.

\noindent At last we input our constructed graph $G$ to the $MaximumWeightedBipartiteMatching$ algorithm, which returns an optimal matching map $E^{'}$ assigning each packet in $V_{1}$ to at most one RU in $V_{2}$ for $n$ future time instants.

\subsection{Pitfalls}

The careful reader would note that the value of the variable $n$ in Algorithm \ref{al:1} could take exceptionally large values if the time periods $T_{0}, T_{1}, \dots T_{l-1}$ are not chosen carefully. Even when the time periods are chosen carefully, a manageable but still sufficiently large value of $n$ would result in an undesirably long execution time since it would result in a very large and possibly dense graph $G$ being passed as input to the $MaximumWeightedBipartiteMatching$ algorithm.

To overcome this drawback, we propose a modified variant of the Optimal Minimize Deadline Profit Scheduling Algorithm in the next section. Needless to say, the modification trades the optimal solution provided by the current algorithm with better execution time.

\section{A Heuristic for the Scheduling Problem}
\label{sec:heuristic}

An simple remedy for the pitfalls discussed for our Optimal Minimize Deadline Profit Scheduling algorithm is to fix the value of the variable $n$ by providing it as input to the algorithm. This has the direct effect of fixing the number of future time instants for which our scheduler generates a schedule. In order to better understand the challenges this remedy brings to the design of the scheduler, consider the following scenario:

Let us assume the following time window $[t_{0}, t_{3n}]$, where $3n + 1 = LCM$ ($T_{0}, T_{1}, \dots T_{l-1}$). A packet $p_{i}$ arrives at time instant $t_{0}$ and has a deadline at $t_{3n}$. Our scheduler is invoked at time instants $t_{0}$, $t_{n}$ and $t_{2n}$ to generate schedules for the considered time window. Now, a node corresponding to packet $p_{i}$ must appear in the graph $G_{1}$ constructed for the first of the three sub-windows, $[t_{0}, t_{n}]$. If $p_{i}$ is not scheduled in this sub-window (perhaps because it had a low profit/priority compared to other packets competing for transmission), a node for it must appear in the graph $G_{2}$ for the second sub-window $[t_{n}, t_{2n}]$. Continuing its bad luck, if the packet is not scheduled even in the second sub-window, a node for it must appear in the graph $G_{3}$ for sub-window $[t_{2n}, t_{3n}]$. Finally, if the packet is not scheduled even in the last sub-window, it must be dropped from the queue. On the other hand, if the packet was scheduled in the first sub-window $[t_{0}, t_{n}]$, then a node corresponding to it must $not$ appear in the graphs $G_{2}$ and $G_{3}$. Hence, we must now maintain a record $X$ of packets that have already been scheduled in an earlier time window.

This also has the indirect effect of modifying the value of the variable $m$ on \textbf{line} $\boldsymbol 4$ of Algorithm \ref{al:1}. We now depend on procedure $getPackets$ to set the value of $m$, which tells the number of packets arriving in the next $n$ time instants. $getPackets$ consults the time periods of packets from $C_{s}$ along with a record $X$ of packets already scheduled at earlier time instants to compute this information. Simply put, it ensures that packets that were scheduled in earlier rounds, do not re-appear as nodes in the graph $G$ being constructed.

However, the most significant effect of the suggested remedy is a deviation from optimality. We discuss this in further detail in Section \ref{sec:deviation}.

\subsection{Modified Mapping Procedure}

We now describe our modifications to the Optimal Minimize Deadline Profit Scheduling Algorithm.

\begin{algorithm}[h!]
$X = \phi$\\
\>\\
def HeuristicMinimizeDeadlineProfitScheduling($C_{s}$, $A_{s}$, $j$, $t_{i}$, $n$):\\
\>Create $t_{s} = \{ t_{i}, t_{i+1}, \dots t_{i+n-1} \}$\\
\>$m = $getPackets($C_{s}$, $X$, $t_{i}$)\\
\>Create $p_{s} = \{ p_{0}, p_{1}, \dots p_{m-1} \}$\\
\>\\
\>$G = <V_{1} \cup V_{2}, E, W> = $ ConstructBipartiteNullGraph($m$, $n*j$)\\
\>\\
\>for each $A \in A_{s}$:\\
\>\>\>\>for each $p \in p_{s}$:\\
\>\>\>\>\>\>\>for each $t \in t_{s}$:\\
\>\>\>\>\>\>\>\>\>\>if $t \in [a_{Ap}, d_{Ap}]$:\\
\>\>\>\>\>\>\>\>\>\>for each $r \in r_{s}$:\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$u_{Ap} = V_{1}.$find($A, p$)\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$v_{tr} = V_{2}.$find($t, r$)\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$E$.add($u_{Ap}, v_{tr}$)\\
\>\>\>\>\>\>\>\>\>\>\>\>\>$W$.add($u_{Ap}, v_{tr}$, $P_{A}$)\\
\>\\
\>$E^{'} = $ MaximumWeightedBipartiteMatching($G$)\\
\>\\
\>for each $A \in A_{s}$:\\
\>\>\>\>for each $p \in p_{s}$:\\
\>\>\>\>\>\>\>if $E^{'}$.isMapped($u_{Ap}$):\\
\>\>\>\>\>\>\>\>\>\>$X$.add(p)\\
\>\\
\>return $E^{'}$\\
\caption{Heuristic Minimize Deadline Profit Scheduling Algorithm}\label{al:2}
\end{algorithm}

Our Heuristic Minimize Deadline Profit Scheduling Algorithm \ref{al:2} has the following differences when compared to the Optimal version.
\begin{itemize}
    \item The number of future time instants $n$ for which a schedule has to be generated is now provided as input.
    \item After $MaximumWeightedBipartiteMatching$ returns the map $E^{'}$, we add a record corresponding to each packet that was assigned an RU into $X$.
    \item The method $getPackets$ now computes the number of packets arriving in the next $n$ time instants by consulting $C_{s}$, $X$ and the current time instant $t_{i}$.
\end{itemize}

\subsection{When Do We Deviate From Optimality?}
\label{sec:deviation}

Consider the following example scenario. We have three applications described by the integer tuples $<T_{i}, s_{i}, d_{i}, P_{i}>$, specifically, $A_{0} = <2, 10, 0, 1>$, $A_{1} = <2, 30, 1, 2>$ and $A_{2} = <2, 100, 1, 3>$. Let, $C_{s} = \{ A_{0}, A_{1}, A_{2} \}$. We set $j = 2$ to represent the $2x242$-tone RU configuration.

We first provide this input to the Heuristic Minimize Deadline Profit Scheduler with $t_{i} = t_{0}$, and $n = 1$ to imply that our scheduler generates a schedule only for the next time instant. Observe what happens over the time window $[t_{0}, t_{1}]$. 

\begin{figure}[h!]
\subfloat[]{\includegraphics[width = 0.24\textwidth]{figs/deviation_1.pdf}}
\subfloat[]{\includegraphics[width = 0.24\textwidth]{figs/deviation_2.pdf}}
  \caption{(a) Graph $G_{1}$ for time instant $t_{0}$, (b) Graph $G_{2}$ for time instant $t_{1}$}
  \label{fig:deviation_herustic}
\end{figure}

At the time instant $t_{0}$, one packet is generated by each application and so $m = 3$. The scheduler generates the graph $G_{1}$ shown in Figure \ref{fig:deviation_herustic} above and gives it as input to the $MaximumWeightedBipartiteMatching$ algorithm, which outputs the matching shown via green edges. A profit of $1$ is incurred since the packet for application $A_{0}$ is dropped.

At time instant $t_{1}$, no new packet arrives, $m = 0$, and so the output $E'$ is empty. No profit is incurred.

We now provide the original input to the Optimal Minimize Deadline Profit Scheduling Algorithm with $t_{i} = t_{0}$ and again observe what happens over the time window $[t_{0}, t_{1}]$.

\begin{figure}[h!]
  \centering
  \captionsetup{type=figure}
    \centering
    \includegraphics[scale=0.5]{figs/deviation_3.pdf}
    \caption{Optimal Packet-to-RU assignment by Optimal Minimize Deadline Profit Scheduler}
   \label{fig:deviation_optimal}
\end{figure}

Clearly, $n = LCM$($T_{0}, T_{1}, T_{2}$) $= LCM$($2, 2, 2$) $= 2$ and $m = 3$. The scheduler generates the graph $G_{3}$ shown in Figure \ref{fig:deviation_optimal} and $MaximumWeightedBipartiteMatching$ generates the matching shown via green edges. No profit is incurred.

One can quickly infer from this example that presence of applications with long packet deadlines and a high packet drop profit along with a small value of the input $n$ cause the Heursitic variant of our scheduler to deviate from optimality. Had we given $n = 2$ as input to our Heuristic Minimize Deadline Profit Scheduler, we would have been provided with the same optimal value of $0$ profit incurred as provided by the Optimal Minimize Deadline Profit Scheduler.

Fortunately, for most practical factory settings, rarely do we encounter applications with relaxed delay tolerances and high packet drop penalties. In most cases, a stringent delay tolerance is itself an indicator of high packet priority. Therefore, we expect our Heuristic scheduler to provide good performance in typical factory environments. With this expectation, in the next section, we evaluate the performance of our scheduler by implementing it and simulating a factory scenario in ns-3.


==> background-extra.tex <==
\iffalse
\subsection{WiFi for Flexible Factory}

There is an increasing demand on industries that manufacture goods to support customized production.
Customized production requires industries to scale up or down the amount of production depending on the demand, availability of raw materials and/or the condition of the machinery \cite{smart-factory}.
With an annual worldwide growth of 13\%, it is expected that such ``flexible factories" would dominate global manufacturing within the next 15 years \cite{market-share}.

A key requirement of such flexible factories is to have sensors to collect data in real-time about the condition of the factory and have actuators that adapt to the conditions \cite{smart-factory}.
Traditionally, such data was collected through wired network protocols such as Industrial Ethernet \cite{industrial-ethernet}.
However, with factories getting more complex, there are hundreds of sensors and actuators that need to be connected.
This makes the process of wiring very expensive and rigid, which makes it important to leverage wireless networks \cite{critical}.


Utilizing wireless network protocols is non-trivial for such industrial networks because of a few reasons.
First, most wireless network protocols are not oriented towards satisfying deadlines or reliability requirements.
Furthermore, unlike traditional networks, industrial networks have different priorities for the packets depending on the application \cite{critical}.
For example, a usage survey by the Flexible Factory Project \cite{noauthor_wireless_nodate} categorized the various wireless applications in current use in factories. Some of the major categories include:
(1) Quality Supervision, (2) Factory Resource Management, (3) Human Safety.
The survey also provides the details of the communication requirements for these applications (summarized in Table \ref{tab:factory-applications}). We observe  that many applications have delay tolerance values lower than a few milliseconds, while others have comparatively relaxed tolerance values of the order of hundreds of milliseconds or more. Furthermore, for some applications, such as human safety monitoring and equipment control, the rate of communication is very high, i.e, once every one or two milliseconds.
These observations make it essential to have a protocol that can be adopted for such requirements.

Although 3GPP envisages the use of private 5G for such critical requirements, their deployment is significantly more expensive than that of WiFi.
Private 5G also requires acquiring of license to operate, making them more difficult to operate for smaller manufacturing units.
Moreover, the recent versions of WiFi, such as WiFi 6 and 7 (IEEE 802.11ax and 802.11be), have centralized the access given to the stations (user devices) to the access point (AP) instead of allowing decentralized access via CSMA/CA.
These standards use orthogonal frequency division multiplexing with multiple access (OFDMA), thus enabling allocation of smaller or higher bandwidths depending on the requirement.
Such utilization of newer WiFi standards for the flexible factory is also envisaged by the WiFi Broadband Alliance, the designers of the WiFi standards \cite{white-paper}.
This requirement motivates us to design an efficient algorithm that provides performance bounds on the delivery of deadline-driven packets.



\subsection{Functioning of Centralized Access of WiFi 6}
\label{sec:central}

The WiFi 6 standard reduces the complexity of the transmitting and receiver devices by restricting the number of available transmission choices ~\cite{11ax-standard}.
It uses transmission units of contiguous orthogonal sub-carriers or tones, called Resource Units (RU).
Depending on the number of contiguous tones, there are six different configurations of the RU's, with the RU's arranged in a hierarchy of increasing bandwidth.
The narrowest RU uses $~2$ MHz ($26$ tones), whereas the widest one uses 160 MHz ($2*996$ tones). There are also configurations which utilize a mix of these widths.
Note that since WiFi 6 allows only transmission of at most $160$ MHz bandwidth, there is a limitation on the number of parallel users depending on the type of RU's used.
Furthermore, each user can use a maximum of one RU at a time.

The centralized nature of WiFi 6 works as follows.
The AP advertises a MU-EDCA (multi-user Enhanced distributed channel access) mode, where it can specify the contention parameters of each station after a transmission \cite{muedca-impact}. In the MU-EDCA procedure, the access point advertises a set of EDCA parameters composed of channel contention parameters and a countdown timer. The stations switch their contention parameters to MU EDCA parameters for a duration specified by the countdown timer. During this time, stations' contention for channel access can be completely suppressed and thus channel access can be completely centralized by relegating all access responsibilities to the access point. This feature can be utilized to counter non-determinism associated with the randomised channel access procedure (DCF/EDCA) employed by stations in a WiFi network which is a primary obstacle to the deployment of WiFi in factory settings.

The transmission opportunity is given to each node at most for a fixed time duration, known as TXOP.
Thus, the parallel OFDMA transmission starts in a completely synchronized manner, but can end at different times. However, in that case, the next parallel transmission can only start when all the clients have finished sending their data.
The next transmission can resume shortly after a previous transmission ends, with the time gap between them being a predefined constant.
Such setting of the MU-EDCA and TXOP parameters enables the AP to control the exact timings of transmission of each station, making the transmission deterministic.

\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{figs/valid-invalid-tx.pdf}
  %  \vspace{-0.1in}
    \caption{Examples of a few legal (subfigures (La)-(Lc)) and illegal (subfigures (Ia)-(Ic)) transmissions with a system of three user devices C1-C3 within a period of three TxOPs (denoted by $\delta$).}
    \label{fig:transmissions}
\end{figure}

Figure \ref{fig:transmissions} illustrates a few cases of legal and illegal transmissions.
In Figure \ref{fig:transmissions}(La), we show that a case of legal transmission where the transmissions have started together, and ended separately.
On the other hand, Figure \ref{fig:transmissions}(Ia) is a case of illegal transmission since C1 starts transmission before C2 and C3 have finished the transmission of previous slot.
In Figure \ref{fig:transmissions}(Lb), the transmissions have all ended before the TXOP, but a new transmission has started immediately, which is legal.
However, the transmissions of Figure \ref{fig:transmissions}(Ib) are illegal, as the transmissions of the second slot last longer than the TXOP.
The third case of legal transmission is shown in Figure \ref{fig:transmissions}(Lc), where in the first slot the user device C3 does not transmit any data, but starts the next transmission after the other user devices complete.
Again, the transmissions of Figure \ref{fig:transmissions}(Ic) are illegal, as the transmissions of C3 have started before those of C1 and C2 have finished.
This shows how the process of parallel transmissions and synchronization work in practice.

% % Thus, a maximum of one RU to each user and provides a specific way of splitting the RU's. The maximum number of RU's of different tones per channel bandwidth is shown in Table~\ref{tbl:maxru}.
% % Each wide RU can be split into two narrower RU's that, in turn, can be split again independently. However, there are exceptions  for $242$ tone and $996$ tone RU's. These are split into $3$ narrower RU's; two $106$ tone RU \& one $26$ tone and two $484$ tone RU \& one $26$ tone respectively. 
% \begin{table}[t!]
% \footnotesize
% \caption{The Maximum Number of RU's for Each Bandwidth~\cite{11ax-standard, tutorial}.
% *$^{+n}$ means "plus n 26-tone RU's"}
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{RU type} & $20$ MHz & $40$ MHz & $80$ MHz & $160 (80+80)$ MHz\\
% \hline
% 26-tone & 9 & 18 & 37 & 74\\
% 52-tone & $4^{+1}$ & $8^{+2}$ & $16^{+5}$ & $32^{+10}$\\
% 106-tone & $2^{+1}$ & $4^{+2}$ & $8^{+5}$ & $16^{+10}$\\
% 242-tone & 1 & 2 & $4^{+1}$ & $8^{+2}$\\
% 484-tone & NA & 1 & $2^{+1}$ & $4^{+2}$\\
% 996-tone & NA & NA & 1 & 2\\
% \hline
% \end{tabular}
% \label{tbl:maxru}
% \vspace{-0.6cm}
% \end{table}

% 802.11ax introduces uplink and downlink OFDMA in WiFi, coordinated by the access point. The standard also introduces a Multi-User (MU) EDCA procedure that allows the access point to tweak the priorities of nodes contending for channel access via an advertised MU EDCA parameter set. The MU EDCA parameter set contains contention window parameters to be used by stations for channel access contention via the EDCA (Enhanced Distributed Channel Access) mechanism, along with a countdown timer.

% Uplink OFDMA transmissions are solicited from the stations by the access point via the downlink transmission of a trigger frame. The trigger carries various transmission related parameters, including station-to-RU mapping related information. Upon reception of the trigger, the stations wait for a SIFS duration before participating in a synchronized uplink OFDMA transmission.
% After successfully performing an uplink OFDMA transmission, the stations change their contention window parameters to the MU EDCA parameters advertised by the access point for a duration specified by a countdown timer. A long value for the MU EDCA countdown timer can completely suppress station contention for channel access in the network. In such a situation, the stations become dependent on uplink OFDMA transmissions solicited by the access point to transmit data. And so, the transmission paradigm for stations shifts from being distributed contention-based, to centralized polling based.

% In a network with station contention completely suppressed, all channel access decisions are made by the access point. This removes the non-determinism associated with randomised channel access schemes such as DCF/EDCA, thus removing a major obstacle limiting WiFi deployment in factory networks. We utilize these features to design a Minimize Deadline Profit scheduler in this work. The scheduler at the access point generates a schedule specifying the station-to-RU mapping for each station. The mapping is transmitted to relevant stations via a downlink trigger frame. A SIFS duration after the trigger is received, the stations perform an uplink OFDMA transmission. Station contention for channel access is completely suppressed via the MU EDCA procedure.
\fi

==> extra.tex <==

\begin{table}[h!]
\footnotesize
    \centering
\begin{tabular}{|p{2.25cm}|p{1cm}|p{0.8cm}|p{1.25cm}|p{0.75cm}|p{0.5cm}|}
    \hline
      \textbf{Application} & \textbf{Time Period (ms)} & \textbf{Size (B)} & \textbf{Delay Tolerance (ms)} & \textbf{Profit} & \textbf{Nodes} \\
     \hline
        \multicolumn{6}{|c|}{Equipment Control} \\
     \hline
        Bottle filling & $1$ & $400$ & $0.5$ & $90$ & $3$ \\
     \hline
      Warehouse & $2$ & $10$ & $1$ & $100$ & $6$ \\
     \hline
        \multicolumn{6}{|c|}{Quality Supervision} \\
     \hline
        Monitoring equipment & $1000$ & $100$ & $1000$ & $50$ & $4$ \\
     \hline
        Detect defect state & $100$ & $500$ & $100$ & $40$ & $10$ \\
     \hline
        \multicolumn{6}{|c|}{Factory Resource Management} \\
     \hline
        Movement analysis & $500$ & $20$ & $500$ & $10$ & $10$ \\
     \hline
        \multicolumn{6}{|c|}{Human Safety} \\
     \hline
        Detect entry in the proximity of a machine & $10$ & $30$ & $2$ & $200$ & $7$ \\    
     \hline
    \end{tabular} 
    \caption{Characteristics of the 40 applications in our Simulated Factory Settings}
    \label{table:5}
\end{table}

% IEEE 802.11ax also introduces the procedure of Multi-User (MU) EDCA (Enhanced Distributed Channel Access)~\cite{muedca-impact}, where distributed contention-based channel access scheme is completely replaced by a centralized scheme. In a centralized scheme, the access point only is in charge of scheduling both uplink and downlink traffic. In the MU-EDCA procedure, the access point advertises a set of EDCA parameters composed of channel contention parameters and a countdown timer. The stations switch their contention parameters to MU EDCA parameters for a duration specified by the countdown timer. During this time, stations' contention for channel access can be completely suppressed and thus channel access can be completely centralized by relegating all access responsibilities to the access point. This feature can be utilized to counter non-determinism associated with the randomised channel access procedure (DCF/EDCA) employed by stations in a WiFi network which is a primary obstacle to the deployment of WiFi in factory settings.
%(4) one user can be allocated to at most one RU.% further there are resthe parallelism allowed by break up of the channels into RU's has to be intelligent used, as smaller RU's also lead to smaller packets. The possible configurations of the RU's are explicitly defined in the standard (details in \S II).
%Furthermore, the transmissions cannot happen completely in parallel, but need to be periodically synchronized to enable the access point to switch to a different RU configuration.

%by enforcing the stations to follow packet transmission schedules provided by the access point via a trigger frame. %Here, we consider the transmission time of a frame is atmost TXOP 
%two different scenarios: (a) case 1: where transmissions are small i.e., $<1$ ms. (b) case 2: transmissions are moderate i.e., less than the TXOP duration $<5$ ms. 
%We show that our scheduler significantly improves the profit obtained due to achieving the deadlines of the applications compared to other deadline-based schedulers.
%{\color{red} Syam : I think `Our contribution' should be more crisp}



==> insights.tex <==
\subsection{Analysis and Insights}

Here, we first discuss the differences between our Minimize Deadline Profit scheduler and the state-of-the-art deadline-based scheduler by Inam et al.\cite{inamullah_will_2020}. (1) The scheduler proposed by \cite{inamullah_will_2020} uses a deadline estimation approach that utilizes the station queue length provided by the buffer status reports collected by the access point from the stations. On the other hand, our scheduler assumes that the access point is already aware of the deadlines for each application running on a station.(2) Once deadlines have been estimated, their scheduler sorts the stations in an earliest-deadline-first order and then performs an exhaustive search over all RU configurations to find the one that results in the least expected packet drops. It utilizes a recursive mathematical expression to estimate the number of packets dropped when the first $m$ sorted stations are assigned the first $m$ RUs (RUs sorted by their size, where $m$ is the number of available RUs) for a given RU configuration. Our Maximize Deadline Profit Scheduler does not perform an exhaustive search since it always chooses an RU configuration that splits the bandwidth into equal sized RUs to maximizes the number of packets that can be transmitted. This choice is justified since we only consider small payloads in our uplink traffic.


Based on the above two differences one can infer that for the small payload and known deadline scenario we are considering, the scheduler by \cite{inamullah_will_2020} would simply sort the stations based on the known deadlines and then assign the first $m$ stations to the first $m$ RUs of the fixed RU configuration input to the scheduler. Thus, their scheduler reduces to a simple Earliest Deadline First (EDF) scheduler.

It is evident from Figures \ref{fig:18_RU} and \ref{fig:4_RU} that our scheduler far outperforms the Earliest Deadline First scheduler for the factory IoT setting. Both the Heuristic and the Optimal variants of our scheduler provide zero packet drops and result in zero profit incurred when the $18\times26$-tone RU configuration is used, even for the $4\times106$-tone RU configuration, a $36.5\%$ reduction in profit is observed compared to EDF. This is a consequence of the fact that our scheduler exploits knowledge of the packet arrival patterns to generate a schedule not just for the subsequent transmission but for several future transmissions.
Similarly, the poor performance of the LRF and NLRF schedulers can be attributed to the fact that their scheduling decisions are based on local instantaneously available information only. Moreover, both the LRF and NLRF schedulers continue to exhibit starvation for certain applications, particularly for the ones with very long time periods.

Another interesting point to note is that neither $Heuristic(10)$ nor $Heuristic(5)$ deviates from the optimal value generated by $Optimal$. This is due to the fact that the our simulation does not include any application with long packet deadlines and high profit, which could cause deviation from Optimality, as explained in Section \ref{sec:deviation}.
Table \ref{table:6} points out that the execution time for the Heuristic Minimize Deadline Profit scheduler is smaller than the number of time instants for which it is generating a schedule ($n = 5$ and $n = 10$ ms). This is a lucky co-incidence, for some settings it is possible that the execution time of the scheduler turns out to be longer than $n$ which would cause the scheduler to finish its scheduling operations before a schedule for the next $n$ time instants is generated. In such a scenario, the suggested remedy is to gain a head-start of $12-18$ ms by generating a schedule for $2$ to $3$ time windows when the \textit{very first} schedule is being generated. Afterwards, schedule generation should proceed in parallel along with scheduling operations at the access point to ensure that a schedule is always available. This approach has the small disadvantage that newly associated stations must wait for $10$ to $20$ ms before a schedule that considers them is generated.


==> problem-statement.tex <==
\section{Notations and Problem Formulation}
\label{sec:model}

%In this section, we formulate our Deadline-based scheduling problem as an Integer Linear Programming Problem.
We first discretize the time units and denote them as $t_0, \ldots, t_n$, and assume that transmissions can start only at the beginning of some $t_i$.
Let each user device generate a set $\bbP$ of packets.

\noindent Let the time axis be divided into discrete time quanta $[t_{0}, t_{1}], [t_{1}, t_{2}] \dots [t_{n-1}, t_{n}]$ of fixed duration $\Delta = 1$ ms. Thus, $t_{i} = i*\Delta$. 

\noindent And, let $m$ packets $p_{0}, p_{1}, \dots p_{m-1}$ be generated by $l$ applications $A_{s} = \{ A_{0}, A_{1}, \dots A_{l-1} \}$ over $n$ time instants $t_{0}, t_{1}, \dots t_{n-1}$. Where, for each time instant, we have $j$ equal sized RUs available $r_{0}, r_{1} \dots r_{j-1}$.

\noindent Moreover, each packet $p_{i}$ has an associated arrival time $a_{i}$ and deadline $d_{i}$. And each wireless application $A_{i}$ is described using the integer tuple $<T_{i}, s_{i}, d_{i}, P_{i}>$, based on the information in Table \ref{table:3}.

\noindent Where, $T_{i}$ is the time period of packet generation/communication rate for the application.\\
$s_{i}$ is the size of the application packets.\\
$d_{i}$ is the delay tolerance for the application packets.\\
$P_{i}$ is the profit/priority of the application packets.

\subsection{Assumptions}
Before we proceed with a concrete formulation of our scheduling problem, it is important to enumerate the assumptions about the nature of our problem: (1) Packet deadlines and arrival patterns known: We assume that the access point is aware of the deadlines and packet arrival patterns of each wireless application deployed in the network. This is a valid assumption in a factory setting where each application has well known characteristics as mentioned in Table \ref{table:4}. (2) Only one application per station: Every station has one and only one application running on it which generates packets according to a configured time period. This assumption is true for most IoT devices which only serve a single function, e.g., transmit data collected from sensors. (3) Packets dropped on expiration of deadline: Whenever a packet's deadline expires, it is immediately dropped from the access point queue. The applications can be easily configured to meet this requirement. (4) No packet queuing at the stations: A new packet for an application is not generated until the last packet's deadline has expired, and the packet has been dropped as a consequence. Mathematically, this means that $T_{i} > d_{i}$ for each application. In this work, we only consider applications that meet this requirement by generating periodic traffic.
    %A fixed resource unit configuration: Since the payload sizes $s_{i}$ are small, the best way to split the bandwidth into resource units (RUs) is to choose a RU configuration that maximizes the number of packets that can be transmitted. For example, for 40 MHz bandwidth, if $20$ packets would arrive for transmission over a time window $[t_{i}, t_{j}]$, choose the $18\times26$-tone resource unit configuration. If $3$ packets arrive, choose the $4\times106$-tone configuration (one resource unit would be wasted in this case). Therefore, as an input to our scheduling problem, we have a fixed RU configuration that is decided based on the number of packets that would be arriving over the considered time window for scheduling. All possible RU configurations are given in Figure \ref{fig:ru_config}.
    (5) Packets arrive only at the fixed time instants: We assume that all applications were started at the beginning of some time instant. This assumption aids in the modelling of our scheduling problem with minimal deviation from reality, since our considered value of $\Delta = 1$ ms is very small.  (6)Same MCS value for all stations: We assume that every station observes similar channel conditions and is thus assigned the same MCS value. This assumption has been made to simplify the design of our scheduler.
    %\item \textbf{Transmissions contained within a time quantum:} Every transmission starts at the beginning of a time quantum and ends before the next time quantum starts. In effect, every transmission is contained within some time quantum and lasts for a maximum duration of $1$ ms. In order to achieve this, we ensure that the transmission duration $\tau$, which is a function of the chosen RU configuration $r$, the MCS value assigned to all stations $m$ and the size of the largest payload in the transmission $s = $ $max$ ($s_{k}$) $\forall k$ ($k$ is the number of stations participating in the transmission), is less than the duration of a time quantum $\Delta$. Mathematically, $\tau(r, m, s) < \Delta$.
  %  \item \textbf{Only one transmission allowed per time quantum:} Even if a transmission ends well before the end of the time quantum in which it was scheduled, the next transmission cannot start until the beginning of the next time quantum. This requirement has been imposed only to aid the design of our scheduler.



%\section{Approximation Algorithm for \pmss} 


%Let $z_{ij}$ denote a transmission that starts at $i$ and ends at $j$. Only transmissions with duration less than equal to TXOP are allowed. In this paper, we take value of TXOP=$5$ ms.\\\\
%if $j - i > 5$ or $j - i \le 0$ then
%\begin{equation}
%    z_{ij} = 0, \forall i, j\\
%\end{equation}

%Let $t$ be any time instant between $[0, T]$. At most one transmission $z_{ij}$ can be active at any given time instant $t$.\\
%\begin{equation}
%    \sum_{[i, j]: t \in [i, j]} z_{ij} \le 1, \forall t\\
%\end{equation}

%if $z_{ij} = 1$, then
%\begin{equation*}
%    \sum_{m = i}^{j} \sum_{n = m + 1}^{m + 5} z_{mn} +  \sum_{n = %j}^{i} \sum_{m = n - 1}^{n - 5} z_{mn} = 0, \forall i, j \\
%\end{equation*}
%where $z_{mn} \neq z_{ij}$

%Let, $x_{kij}$ denote packet $k$ assigned to transmission [$i, j$], then

%\begin{equation}
%    \textbf{OR}_{k} \ x_{kij} = z_{ij}, \forall i, j \\
%\end{equation}

%\begin{equation}
%    \sum_{k} x_{kij} \le k * z_{ij}, \forall i, j \\
%\end{equation}

%Let $\lambda_{k}$ denote that the packet is scheduled for transmission in its arrival $a_{k}$ and deadline $d_{k}$ interval, then

%\begin{equation}
%    \sum_{i = a_{k}}^{d_{k} - 1} \sum_{j = i}^{d_{k}} x_{kij} = \lambda_{k}, \forall k \\
%\end{equation}

%Let $m$ RUs be available for scheduling in any transmission, then at most $m$ packets can be scheduled in any transmission.

%\begin{equation}
%    \sum_{k} x_{kij} \le m, \forall i, j \\
%\end{equation}

%Let $t_{k}$ represent the duration of the transmission for packet $k$, then packet $k$ cannot be scheduled in an interval [$i, j$], if the duration of the packet is longer than the duration of the interval.\\\\
%if $i + t_{k} > j$, then
%\begin{equation}
%    x_{kij} = 0, \forall k, i, j \\
%\end{equation}

%Finally,

%\begin{equation}
%    \textbf{Minimize } \sum_{k} (1 - \lambda_{k})p_{k}, \forall k\\
%\end{equation}


%In general, ILPs are NP-Hard, thus, it is undesirable to solve the formulated ILP via conventional optimization solvers. Therefore, in the next section, we propose a polynomial time algorithm to solve the scheduling problem.


==> related-not-used.tex <==
\section{Background and Related Work}
\label{sec:rel}
The IEEE 802.11ax standard~\cite{11ax-standard} restricts assignment of maximum of one RU to each user and provides a specific way of splitting the RUs. The maximum number of RUs of different tones per channel bandwidth is shown in Table~\ref{tbl:maxru}.
Each wide RU can be split into two narrower RUs that, in turn, can be split again independently. However, there are exceptions  for $242$ tone and $996$ tone RUs. These are split into $3$ narrower RUs; two $106$ tone RU \& one $26$ tone and two $484$ tone RU \& one $26$ tone respectively. 
\begin{table}[t!]
\footnotesize
\caption{The Maximum Number of RUs for Each Bandwidth~\cite{11ax-standard, tutorial}.
*$^{+n}$ means "plus n 26-tone RUs"}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{RU type} & $20$ MHz & $40$ MHz & $80$ MHz & $160 (80+80)$ MHz\\
\hline
26-tone & 9 & 18 & 37 & 74\\
52-tone & $4^{+1}$ & $8^{+2}$ & $16^{+5}$ & $32^{+10}$\\
106-tone & $2^{+1}$ & $4^{+2}$ & $8^{+5}$ & $16^{+10}$\\
242-tone & 1 & 2 & $4^{+1}$ & $8^{+2}$\\
484-tone & NA & 1 & $2^{+1}$ & $4^{+2}$\\
996-tone & NA & NA & 1 & 2\\
\hline
\end{tabular}
\label{tbl:maxru}
\vspace{-0.6cm}
\end{table}

Now, we discuss the prior work related to the SRA problem of IEEE 802.11ax.
This has gained a lot of attention in recent times~\cite{icc-2018, mutax-pimrc17, freq-heu,recursive-infocom18, infocom2020j, throughput-max, deepmux}, where the authors formulate this as an optimization problem and propose various solutions for the same. In~\cite{throughput-max}, the authors use an optimization solvers for solving their optimization problem. In~\cite{deepmux}, the authors employ  deep neural
networks (DNNs) to solve the SRA problem. In~\cite{icc-2018, mutax-pimrc17, freq-heu,recursive-infocom18, infocom2020j} the authors propose various algorithms to solve the SRA problem. Below, we discuss them in details.


 The uplink SRA problem has been considered in~\cite{icc-2018, mutax-pimrc17, freq-heu}. The authors consider a generic utility function of maximizing the sum. They showcase how various popular scheduling algorithms proposed for LTE can be adapted for IEEE 802.11ax as well, such as Sum Rate (SR), Proportional Fair (PF)  and Shortest Remaining Processing Time (SRPT) etc. It uses the Hungarian Algorithm for optimal assignment of resources to the user for a fixed RU configuration and MCS (Modulation and Coding Scheme). They exhaustively search over all possible RU configurations and MCS set to solve the SRA problem subject to the maximizing the sum utility function. The SRA algorithm needs to run at an AP in real time for each OFDMA transmission. Hence, such enumerative strategies are not practical, specifically for high bandwidth configuration. The authors~\cite{deadline}  propose a way of estimating the deadlines of packets and propose a deadline-based uplink OFDMA scheduling using  such enumerative strategies.

The authors in~\cite{recursive-infocom18}  consider the problem of assignment of RUs to users and user groups with the goal of maximizing the weighted sum rate.
The authors propose an optimal divide and conquer based algorithm. However their algorithm and its proof of optimality require the crucial assumption that a user or user group can be assigned to multiple RUs, which violates an important restriction in 802.11ax. Further, the core strategy of their algorithm is to split one RU in to exactly two smaller RUs, thereby creating a `tree structure' which makes it amenable to a divide and conquer strategy. However, such a specific splitting strategy might potentially miss several other options in the feasible RU configuration space. 
The authors propose two practical  heuristics - Greedy and Recursive. These algorithms follow the standard restriction of the assignment of one RU to a user or user group. However, the authors do not prove any performance bound for these two algorithms. As we shall show in our evaluation,  the best of these two i.e., the recursive one, provides sub-optimal performance. The authors extended~\cite{infocom2020j} this work for a generic objective of  maximizing the weighted sum. 
We take their recursive algorithm in this paper as our baseline and call it \recursivenospace. 


==> removed-usecase-text.tex <==
\noindent
\textbf{Use Case-2 (UC-2):} Next, we simulate M2M (Machine-to-Machine) traffic with small, infrequent uplink traffic with stringent delay requirements. As considered in~\cite{usecase2-paper}, there are four different classes of delay-sensitive M2M traffic (A, B, C, and D) with different uplink delay budgets. Table.~\ref{usecase2-table} summarises the attributes of these traffic classes. %The inter-arrival times of requests have an exponential distribution with a mean arrival rate specified in the table. 
We consider the uplink delay budget as the deadline. Here again, we consider the same profit for all categories A, B, C, and D.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.6cm}|p{2cm}|p{0.5cm}|p{1.2cm}|p{0.85cm}|p{1cm}|}
    \hline
        \textbf{Appl.} & \textbf{Gen. rate (pkts/s)}  & \textbf{Size (B)} & \textbf{Deadline (ms)} & \textbf{Profit} & \textbf{\# Nodes} \\ \hline
        A & $150$ & $32$ & $20$ & $10$ & $10$ \\ \hline
        B & $5 \times U (3, 6)$ & $32$ & $40$ & $10$ & $10$ \\ \hline
        C & $7.5 \times U(5, 20)$ & $32$ & $60$ & $10$ & $10$ \\ \hline
        D & $75 \times U(1, 3)$ & $32$ & $80$ & $10$ & $10$ \\ \hline
    \end{tabular}
    \caption{Use Case-2 (UC-2) Application Characteristics~\cite{usecase2-paper}}
    \label{usecase2-table}
    %\vspace{-0.2in}    
\end{table}
\subsubsection{Use Case-2}
\begin{figure}[!ht]
\subfloat[]{\includegraphics[width = 0.25\textwidth]{graphs/evalUC2.pdf}}
\subfloat[]{\includegraphics[width = 0.25\textwidth]{graphs/percentageDroppedUC2.pdf}}
%\vspace{-0.5cm}
\caption{Use Case-2 (UC-2): Evaluation results for LSDS, LSDSF, EDF, LRF, and NLRF; (a) Ratio of profit obtained to total profit, (b) Percentage of total packets and critical packets dropped.}
\label{usecase2-profit}
%\vspace{-0.4cm}
\end{figure}
Figure \ref{usecase2-profit} shows the ratio for UC-2. In this case, as the total load in the network is less than $2$ Mbps, \lsds was able to schedule all packets within their deadline obtaining a profit ratio of $1$. Since the packet size here is small, having small RU's is sufficient to schedule the packets and thus, fixed \lsdsf gives identical results as \lsds. Similarly, LRF and EDF also show identical results. 
%Further,  NLRF suffers by prioritizing higher deadline applications with the same profit. 
Further, in this case the applications with higher delay tolerance i.e., application C and D have a packet generation rate similar to A and B. Hence, the difference in performance between these three benchmarks is marginal. 

